Exact Matching and the Top-k Perfect Matching Problem

The aim of this note is to provide a reduction of the Exact Matching problem to the Top-$k$ Perfect Matching Problem. Together with earlier work by El Maalouly, this shows that the two problems are polynomial-time equivalent. The Exact Matching Problem is a well-known 40 years old problem for which a randomized, but no deterministic poly-time algorithm has been discovered. The Top-$k$ Perfect Matching Problem is the problem of finding a perfect matching which maximizes the total weight of the $k$ heaviest edges contained in it.

==> Introduction.tex <==
\section{Introduction}
%While the above results only guarantee XP-algorithms for EM parameterized by (bipartite) independence number, we also make progress on designing corresponding FPT-algorithms in which the exponent in the running time is independent of the independence number. This is summarized by the following partial result, which finds a perfect matching with almost $k$ red edges in FPT-time parameterized by independence number. 

%\begin{theorem} %\label{th:almostFPT}
%There is a deterministic algorithm which given a graph of independence number $\alpha$ either concludes that there exists no perfect matching with exactly $k$ red edges, or outputs a perfect matching with either $k-1$ or $k$ red edges and runs in time $f(\alpha)poly(n)$.
%\end{theorem}

%\vspace{1cm}
In the \emph{Exact Matching Problem}, we are given a graph $G$ together with a fixed coloring of its edges in two colors (red and blue). 
The question is, for a given integer $k$, to decide whether there exists a perfect matching $M$ of $G$ with the additional property that exactly $k$ of the edges of the perfect matching $M$ are red. Clearly, if we have the special case that all edges of the graph are red and $k=n/2$\footnote{$n$ is the number of vertices in the input graph.}, then this problem is simply to decide whether there exists a perfect matching in the graph. However, when the coloring of the edges is heterogeneous, the problem difficulty increases significantly. 


Papadimitriou and Yannakakis~\cite{papadimitriou1982complexity} initially introduced the exact matching problem (denoted from now on by EM) in 1982. They conjectured EM to be NP-hard. This conjecture is still open today. However, a randomized polynomial-time algorithm solving the problem was described by Mulmuley, Vazirani and Vazirani in 1987 in the course of their celebrated isolation lemma~\cite{mulmuley1987matching}. Given standard complexity theoretic hypotheses, this makes it unlikely for EM to be NP-hard. Despite the existence of a polynomial-time randomized algorithm, as of today it is still not known whether EM can also be solved in deterministic polynomial time. The algorithm of Mulmuley et al.\ uses polynomial identity testing and is based on the Schwartz-Zippel Lemma~\cite{schwartz,zippel}, which has resisted all attempts of derandomization so far. Indeed, EM is one of the few natural problems which has a randomized polynomial-time algorithm (i.e.\ it is contained in the complexity class \textsc{\textsc{NP}}) but for which it is not known whether it admits a deterministic polynomial-time algorithm (i.e.\ it is contained in $\textsc{P}$). It is a major open conjecture that \textsc{RP}=\textsc{P}, and so EM becomes a natural candidate to test this hypothesis.

For this reason, EM has been cited in several papers as an open problem. This includes recent breakthrough papers such as the seminal work on the parallel computation complexity of the matching problem~\cite{svensson2017matching}, works on planarizing gadgets for perfect matchings~\cite{gurjar2012planarizing}, works on budgeted, color bounded, or constrained matching problems~\cite{berger2011budgeted,mastrolilli2012constrained,mastrolilli2014bi,stamoulis2014approximation,kelk2019integrality}, on multicriteria optimization problems~\cite{grandoni2010optimization} and on matroid intersection problems~\cite{camerini1992random}.
It is further known that several different problems relate directly or indirectly to EM. The following is a non-exhaustive list of examples: EM is polynomial-time equivalent to the DNA sequencing problem~\cite{blazewicz2007polynomial}. EM is equivalent to a variant of the problem of finding a solution of a binary linear equation system with small hamming weight \cite{arvind2016solving}. EM can be reduced to a special case of the recoverable robust assignment problem \cite{fischer2020investigation}.

\textbf{Previous work.}
Progress in finding deterministic algorithms for EM (and therefore finding positive evidence for the conjecture P=RP) has only been made for restricted graph classes: It is known that EM can be solved in determinisitic polynomial time for planar and more generally $K_{3,3}$-minor free graphs~\cite{yuster2012almost}, as well as graphs of bounded genus~\cite{genus}. These works use Pfaffian orientations to derandomize the algebraic technique from \cite{mulmuley1987matching}. EM can also be solved for graphs of bounded treewidth using Courcelle's meta-theorem \cite{courcelle}. In contrast to these classes of sparse graphs, EM on dense graphs seems to be even harder: Already solving the problem on complete graphs and complete bipartite graphs is highly nontrivial. In fact, at least 4 articles just dealing with this special case have appeared in the literature \cite{karzanov1987maximum,yi2002matchings,geerdes,gurjar2017exact}.
Recent work~\cite{elmaalouly_et_al:LIPIcs.MFCS.2022.46} made a step forward by showing how to solve EM on graphs of constant independence number\footnote{The \emph{independence number} of a graph $G$ is defined as the largest number $\alpha$ such that $G$ contains an \emph{independent set} of size $\alpha$.} $\alpha$ and bipartite graphs of constant bipartite independence number\footnote{The \emph{bipartite independence number} of a bipartite graph $G$ equipped with a bipartition of its vertices is defined as the largest number $\beta$ such that $G$ contains a \emph{balanced independent set} of size $2\beta$, i.e., an independent set using exactly $\beta$ vertices from both color classes.} $\beta$, thus generalizing previous results for complete  and complete bipartite graphs which correspond to the special cases $\alpha=1$ and $\beta=0$. 
They presented an XP-algorithm, i.e.\ an algorithm running in time $O(n^{f(\alpha)})$, for the problem. The existence of an FPT algorithm, i.e.\ an algorithm with running time $f(\alpha)n^{O(1)}$, was left as an open question. To the best of our knowledge, these are the only results from the last 40 years showing that EM can be solved in deterministic poly-time for restricted graph classes.

 Another direction of progress towards solving EM is the study of relaxed versions of it. A first such relaxation would be to lift the requirement for a perfect matching. In \cite{yuster2012almost}, however, it was shown that there is a simple deterministic polynomial time algorithm such that given a "Yes" instance of EM, computes an \emph{almost} perfect matching (i.e. of size at least $\frac{n}{2}-1$) containing $k$ red edges. This result is as close to optimal as possible for this type of relaxation. The study of the other type of relaxation, i.e. relaxing the color constraints, was only recently initiated in \cite{elmaalouly2022exacttopk}. It was shown that there is a deterministic polynomial time algorithm which given a "Yes"-instance of EM outputs a perfect matching with $k'$ red edges, such that $k/2 \leq k' \leq 3k/2$. 

\textbf{Exact matchings modulo 2.} A crucial tool in this paper is to consider matchings with $k'$ red edges, where $k' \equiv_2 k$, that is, matchings of the correct parity. Let $r(M)$ denote the number of red edges in a matching $M$. We define the problem \emph{Correct Parity Matching} (CPM), where given a red-blue edge-colored graph and an integer $k$, the goal is to find a perfect matching $M$ such $r(M) \equiv_2 k$. Note that parity problems (and more general congruency-constrained problems) have been studied in the context of other graph algorithms \cite{hemaspaandra2004complexity,nagele2019submodular}, but we are not aware of prior parity-constrained results for the perfect matching problem in general graphs. A more challenging version of the problem, \emph{Bounded Correct Parity Matching} (BCPM), requires to find a perfect matching $M$ such that $r(M) \equiv_2 k$ \emph{and} $r(M) \leq k$. %Note that the two problems are not equivalent: In BCPM, we have that additionally $r(M)$ is bounded by $k$.



\textbf{Our results.} From now on, when we say that an algorithm has polynomial running time, we mean a deterministic algorithm, whose running time is bounded by $\text{poly}(n)$, even if $\alpha, \beta, k$ are not bounded by a constant. We show in this paper how the problem BCPM can be used to solve EM. Precisely, our results are the following:
\begin{itemize}
    \item We show that EM reduces to BCPM in FPT time parameterized by $\alpha$ in the following sense: There exists an algorithm, which performs two oracle calls to BCPM, and solves EM on general graphs, in running time $f(\alpha)n^{O(1)}$. (The result holds analogously for the bipartite independence number $\beta$). Without access to the BCPM oracle, the algorithm outputs a perfect matching with either $k-1$ or $k$ red edges or deduces that the answer of the given EM-instance is "No". (\Cref{sec:reduction-EM-BCPM}.)
     \item CPM can be solved in polynomial time for all graphs. (\Cref{sec:correct-parity-general})
    \item On bipartite graphs, the more difficult problem BCPM can be solved in polynomial time. (\Cref{sec:BCPM-bipartite}.)
    \item As a consequence, there is an FPT algorithm parameterized by $\beta$ which solves EM on bipartite graphs.
\end{itemize}
